Prediction-Coherent LSTM-based Recurrent Neural Network for Safer Glucose Predictions in Diabetic People

In the context of time-series forecasting, we propose a LSTM-based recurrent neural network architecture and loss function that enhance the stability of the predictions. In particular, the loss function penalizes the model, not only on the prediction error (mean-squared error), but also on the predicted variation error. We apply this idea to the prediction of future glucose values in diabetes, which is a delicate task as unstable predictions can leave the patient in doubt and make him/her take the wrong action, threatening his/her life. The study is conducted on type 1 and type 2 diabetic people, with a focus on predictions made 30-minutes ahead of time. First, we confirm the superiority, in the context of glucose prediction, of the LSTM model by comparing it to other state-of-the-art models (Extreme Learning Machine, Gaussian Process regressor, Support Vector Regressor). Then, we show the importance of making stable predictions by smoothing the predictions made by the models, resulting in an overall improvement of the clinical acceptability of the models at the cost in a slight loss in prediction accuracy. Finally, we show that the proposed approach, outperforms all baseline results. More precisely, it trades a loss of 4.3\% in the prediction accuracy for an improvement of the clinical acceptability of 27.1\%. When compared to the moving average post-processing method, we show that the trade-off is more efficient with our approach.

==> 2-LiteratureReview.tex <==
\section{Literature Review}

The goal of this section is to review the major studies in glucose prediction. For more details, the reader can look at the extensive review by Oviedo \textit{et al.} \cite{oviedo2017review}.

Traditionally, the autoregressive (AR) model and its derivatives are widely used in predicting future glucose values. Sparacino \textit{et al.} demonstrated the ability of the AR model to predict glucose 30 and 45 minutes ahead of time (prediction horizon, PH, of 30 and 45 minutes respectively) in a cohort of type 1 diabetic people \cite{sparacino2007glucose}. In 2009, Eren-Oruklu \textit{et al.} proposed a dynamic adaptation of the parameters of AR and AR with moving average (ARMA) models to account for the most recent glucose dynamics \cite{eren2009estimation}. St\r{a}hl \textit{et al.} explored the use of compartmental models to input CHO and insulin dynamics into an ARMA with exogenous inputs (ARMAX) model \cite{stahl2008short}. 

However, due to their inherent simplicity, the AR models have recently fallen out of favor for more complex regression models. Georga \textit{et al.} explored the use of support vector regression (SVR) in predicting glucose up to 120 minutes ahead of time in type 1 diabetes \cite{georga2013multivariate}. Valletta \textit{et al.} proposed the use of Gaussian processes to include a measure of the physical activity of type 1 diabetic patients into the predictive models \cite{valletta2009gaussian}.

More recently, we have witnessed a shift towards the use of neural-network-based solutions. In 2012, Daskalaki \textit{et al.} demonstrated the superiority of feed-forward neural networks (FFNN) compared to AR models using a virtual type 1 diabetic population (PH of 30 and 45 minutes) \cite{daskalaki2012real}. In 2015, Zarkogianni \textit{et al.} studied different types of neural networks (feed-forward neural networks, self-organizing maps, neuro-fuzzy neural networks) for the prediction of glucose up to 120 minutes ahead of time \cite{zarkogianni2015comparative}. Zecchin \textit{et al.} showed the importance of using insulin and carbohydrate (CHO) information as inputs to predictive models, and in particular neural networks (jump feed-forward) to enhance the predictions at a PH up to 60 minutes \cite{zecchin2016much}. Georga \textit{et al.} studied the use of extreme learning machine models in short-term (PH of 30 minutes) type 1 diabetes glucose prediction \cite{georga2015online}. Finally, recurrent neural networks (RNN) have shown a lot of interest in the field \cite{zarkogianni2011insulin}, and in particular those with long short-term memory (LSTM) units \cite{mirshekarian2017using,debois2018study}.

Most of the studies use the continuous glucose-error grid analysis (CG-EGA) to evaluate the clinical acceptability of glucose predictive models \cite{eren2009estimation,zarkogianni2011insulin,daskalaki2012real,georga2013multivariate,zarkogianni2015comparative,debois2018study,oviedo2017review}. The CG-EGA assesses the clinical acceptability of a glucose prediction based on two components: the accuracy of the glucose prediction and the accuracy of the predicted glucose variation. Most of the models are trained to minimize the mean squared error, and therefore to maximize the accuracy of glucose predictions. However, the accuracy of the predicted variations is not taken into account when training the models, hurting the clinical acceptability of the models. This motivates the idea of building a model that is trained to both have a good glucose prediction accuracy and a good predicted glucose variation accuracy.

==> tables/preprocessing.tex <==
\begin{table*}
    \caption{Number of days and anomalies removed per dataset during its preprocessing (mean $\pm$ standard deviation across the subjects of the given dataset).}
    \label{table:preprocessing}
    \begin{tabularx}{\linewidth}{C|C|C|C|C|C}
        \toprule
        \multirow{2}{*}{\textbf{Dataset}}  & \multicolumn{2}{c|}{\textbf{Days}} & \multicolumn{3}{c}{\textbf{Anomalies removed per iteration}}\\
        &  \textit{Removed} & \textit{Remaining} & \textit{1st} & \textit{2nd} & \textit{3rd}\\
        \midrule
        Ohio  & $15.83 \pm 3.18$ & $38.5 \pm 4.82$ & $6.33 \pm 2.56$ & $1.17 \pm 1.86$ & $0.0 \pm 0.0$\\
        IDIAB  & $2.4 \pm 0.8$ & $29.4 \pm 1.62$ & $21.2 \pm 3.43$ & $8.4 \pm 4.13$ & $2.6 \pm 3.26$\\
         \bottomrule
    \end{tabularx}
\end{table*}

==> tables/results_IDIAB.tex <==
\begin{table*}
    \caption{General performances of the models with mean $\pm$ standard deviation across the IDIAB type-2 diabetic subjects.}
    \label{table:general_results}
    \begin{tabularx}{\linewidth}{l||C|C|C|C|C}
        \toprule
        \multicolumn{6}{c}{\textbf{IDIAB Dataset}}\\
        \toprule
        \multirow{3}{*}{\textbf{Models}} &  \multirow{3}{*}{\textbf{RMSE}} & \multirow{3}{*}{\textbf{dRMSE}} &  \multicolumn{3}{c}{\textbf{CG-EGA}} \\
        & & & Accurate & Benign & Erroneous \\
        & & & Predictions & Errors & Predictions \\
         \midrule
         \multicolumn{6}{c}{\textit{Prediction Horizon = 30 minutes}}\\
         \midrule
         \textcolor{cyan}{\textbf{SNN}} & \textbf{48.47} {$\pm$} 10.02 & \textbf{5.12} $\pm$ 1.14 &  \textbf{68.31} $\pm$ 7.13 & \textbf{19.94} $\pm$ 4.88 & \textbf{11.75} $\pm$ 3.40 \\
         \textcolor{cyan}{\textbf{LSTM}} & \textbf{42.30} $\pm$ 7.13 & \textbf{8.76} $\pm$ 1.33 & \textbf{73.62} $\pm$ 3.45 & \textbf{20.32} $\pm$ 2.11 & \textbf{6.05} $\pm$ 1.86\\
         \textcolor{cyan}{\textbf{TO-SNN}} & \textbf{37.79} $\pm$ 6.11 & \textbf{7.64} $\pm$ 0.79 & \textbf{73.99} $\pm$ 3.14 & \textbf{21.06} $\pm$ 1.99 & \textbf{4.95} $\pm$ 1.80 \\
         \textcolor{cyan}{\textbf{TO-LSTM}} & \textbf{37.79} $\pm$ 6.11 & \textbf{7.64} $\pm$ 0.79 & \textbf{73.99} $\pm$ 3.14 & \textbf{21.06} $\pm$ 1.99 & \textbf{4.95} $\pm$ 1.80 \\
         \midrule
         \multicolumn{6}{c}{\textit{Prediction Horizon = 60 minutes}}\\
         \midrule
         \textcolor{cyan}{\textbf{SNN}} & \textbf{48.47} {$\pm$} 10.02 & \textbf{5.12} $\pm$ 1.14 &  \textbf{68.31} $\pm$ 7.13 & \textbf{19.94} $\pm$ 4.88 & \textbf{11.75} $\pm$ 3.40 \\
         \textcolor{cyan}{\textbf{LSTM}} & \textbf{42.30} $\pm$ 7.13 & \textbf{8.76} $\pm$ 1.33 & \textbf{73.62} $\pm$ 3.45 & \textbf{20.32} $\pm$ 2.11 & \textbf{6.05} $\pm$ 1.86\\
         \textcolor{cyan}{\textbf{TO-SNN}} & \textbf{37.79} $\pm$ 6.11 & \textbf{7.64} $\pm$ 0.79 & \textbf{73.99} $\pm$ 3.14 & \textbf{21.06} $\pm$ 1.99 & \textbf{4.95} $\pm$ 1.80 \\
         \textcolor{cyan}{\textbf{TO-LSTM}} & \textbf{37.79} $\pm$ 6.11 & \textbf{7.64} $\pm$ 0.79 & \textbf{73.99} $\pm$ 3.14 & \textbf{21.06} $\pm$ 1.99 & \textbf{4.95} $\pm$ 1.80 \\
         \midrule
         \multicolumn{6}{c}{\textit{Prediction Horizon = 120 minutes}}\\
         \midrule
         \textcolor{cyan}{\textbf{SNN}} & \textbf{48.47} {$\pm$} 10.02 & \textbf{5.12} $\pm$ 1.14 &  \textbf{68.31} $\pm$ 7.13 & \textbf{19.94} $\pm$ 4.88 & \textbf{11.75} $\pm$ 3.40 \\
         \textcolor{cyan}{\textbf{LSTM}} & \textbf{42.30} $\pm$ 7.13 & \textbf{8.76} $\pm$ 1.33 & \textbf{73.62} $\pm$ 3.45 & \textbf{20.32} $\pm$ 2.11 & \textbf{6.05} $\pm$ 1.86\\
         \textcolor{cyan}{\textbf{TO-SNN}} & \textbf{37.79} $\pm$ 6.11 & \textbf{7.64} $\pm$ 0.79 & \textbf{73.99} $\pm$ 3.14 & \textbf{21.06} $\pm$ 1.99 & \textbf{4.95} $\pm$ 1.80 \\
         \textcolor{cyan}{\textbf{TO-LSTM}} & \textbf{37.79} $\pm$ 6.11 & \textbf{7.64} $\pm$ 0.79 & \textbf{73.99} $\pm$ 3.14 & \textbf{21.06} $\pm$ 1.99 & \textbf{4.95} $\pm$ 1.80 \\
         \bottomrule
    \end{tabularx}
\end{table*}

==> tables/results_Ohio.tex <==
\begin{table*}
    \caption{General performances of the models with mean $\pm$ standard deviation across the Ohio type-1 diabetic subjects.}
    \label{table:general_results}
    \begin{tabularx}{\linewidth}{l||C|C|C|C|C}
        \toprule
        \multicolumn{6}{c}{\textbf{Ohio Dataset}}\\
        \toprule
        \multirow{3}{*}{\textbf{Models}} &  \multirow{3}{*}{\textbf{RMSE}} & \multirow{3}{*}{\textbf{dRMSE}} &  \multicolumn{3}{c}{\textbf{CG-EGA}} \\
        & & & Accurate & Benign & Erroneous \\
        & & & Predictions & Errors & Predictions \\
         \midrule
         \multicolumn{6}{c}{\textit{Prediction Horizon = 30 minutes}}\\
         \midrule
         \textcolor{cyan}{\textbf{SNN}} & \textbf{48.47} {$\pm$} 10.02 & \textbf{5.12} $\pm$ 1.14 &  \textbf{68.31} $\pm$ 7.13 & \textbf{19.94} $\pm$ 4.88 & \textbf{11.75} $\pm$ 3.40 \\
         \textcolor{cyan}{\textbf{LSTM}} & \textbf{42.30} $\pm$ 7.13 & \textbf{8.76} $\pm$ 1.33 & \textbf{73.62} $\pm$ 3.45 & \textbf{20.32} $\pm$ 2.11 & \textbf{6.05} $\pm$ 1.86\\
         \textcolor{cyan}{\textbf{TO-SNN}} & \textbf{37.79} $\pm$ 6.11 & \textbf{7.64} $\pm$ 0.79 & \textbf{73.99} $\pm$ 3.14 & \textbf{21.06} $\pm$ 1.99 & \textbf{4.95} $\pm$ 1.80 \\
         \textcolor{cyan}{\textbf{TO-LSTM}} & \textbf{37.79} $\pm$ 6.11 & \textbf{7.64} $\pm$ 0.79 & \textbf{73.99} $\pm$ 3.14 & \textbf{21.06} $\pm$ 1.99 & \textbf{4.95} $\pm$ 1.80 \\
         \midrule
         \multicolumn{6}{c}{\textit{Prediction Horizon = 60 minutes}}\\
         \midrule
         \textcolor{cyan}{\textbf{SNN}} & \textbf{48.47} {$\pm$} 10.02 & \textbf{5.12} $\pm$ 1.14 &  \textbf{68.31} $\pm$ 7.13 & \textbf{19.94} $\pm$ 4.88 & \textbf{11.75} $\pm$ 3.40 \\
         \textcolor{cyan}{\textbf{LSTM}} & \textbf{42.30} $\pm$ 7.13 & \textbf{8.76} $\pm$ 1.33 & \textbf{73.62} $\pm$ 3.45 & \textbf{20.32} $\pm$ 2.11 & \textbf{6.05} $\pm$ 1.86\\
         \textcolor{cyan}{\textbf{TO-SNN}} & \textbf{37.79} $\pm$ 6.11 & \textbf{7.64} $\pm$ 0.79 & \textbf{73.99} $\pm$ 3.14 & \textbf{21.06} $\pm$ 1.99 & \textbf{4.95} $\pm$ 1.80 \\
         \textcolor{cyan}{\textbf{TO-LSTM}} & \textbf{37.79} $\pm$ 6.11 & \textbf{7.64} $\pm$ 0.79 & \textbf{73.99} $\pm$ 3.14 & \textbf{21.06} $\pm$ 1.99 & \textbf{4.95} $\pm$ 1.80 \\
         \midrule
         \multicolumn{6}{c}{\textit{Prediction Horizon = 120 minutes}}\\
         \midrule
         \textcolor{cyan}{\textbf{SNN}} & \textbf{48.47} {$\pm$} 10.02 & \textbf{5.12} $\pm$ 1.14 &  \textbf{68.31} $\pm$ 7.13 & \textbf{19.94} $\pm$ 4.88 & \textbf{11.75} $\pm$ 3.40 \\
         \textcolor{cyan}{\textbf{LSTM}} & \textbf{42.30} $\pm$ 7.13 & \textbf{8.76} $\pm$ 1.33 & \textbf{73.62} $\pm$ 3.45 & \textbf{20.32} $\pm$ 2.11 & \textbf{6.05} $\pm$ 1.86\\
         \textcolor{cyan}{\textbf{TO-SNN}} & \textbf{37.79} $\pm$ 6.11 & \textbf{7.64} $\pm$ 0.79 & \textbf{73.99} $\pm$ 3.14 & \textbf{21.06} $\pm$ 1.99 & \textbf{4.95} $\pm$ 1.80 \\
         \textcolor{cyan}{\textbf{TO-LSTM}} & \textbf{37.79} $\pm$ 6.11 & \textbf{7.64} $\pm$ 0.79 & \textbf{73.99} $\pm$ 3.14 & \textbf{21.06} $\pm$ 1.99 & \textbf{4.95} $\pm$ 1.80 \\
         \bottomrule
    \end{tabularx}
\end{table*}

==> tables/results_T1DMS.tex <==
\begin{table*}
    \caption{General performances of the models with mean $\pm$ standard deviation across the T1DMS virtual type-1 diabetic subjects.}
    \label{table:general_results}
    \begin{tabularx}{\linewidth}{l||C|C|C|C|C}
        \toprule
        \multicolumn{6}{c}{\textbf{T1DMS Dataset}}\\
        \toprule
        \multirow{3}{*}{\textbf{Models}} &  \multirow{3}{*}{\textbf{RMSE}} & \multirow{3}{*}{\textbf{dRMSE}} &  \multicolumn{3}{c}{\textbf{CG-EGA}} \\
        & & & Accurate & Benign & Erroneous \\
        & & & Predictions & Errors & Predictions \\
         \midrule
         \multicolumn{6}{c}{\textit{Prediction Horizon = 30 minutes}}\\
         \midrule
         \textcolor{cyan}{\textbf{SNN}} & \textbf{48.47} {$\pm$} 10.02 & \textbf{5.12} $\pm$ 1.14 &  \textbf{68.31} $\pm$ 7.13 & \textbf{19.94} $\pm$ 4.88 & \textbf{11.75} $\pm$ 3.40 \\
         \textcolor{cyan}{\textbf{LSTM}} & \textbf{42.30} $\pm$ 7.13 & \textbf{8.76} $\pm$ 1.33 & \textbf{73.62} $\pm$ 3.45 & \textbf{20.32} $\pm$ 2.11 & \textbf{6.05} $\pm$ 1.86\\
         \textcolor{cyan}{\textbf{TO-SNN}} & \textbf{37.79} $\pm$ 6.11 & \textbf{7.64} $\pm$ 0.79 & \textbf{73.99} $\pm$ 3.14 & \textbf{21.06} $\pm$ 1.99 & \textbf{4.95} $\pm$ 1.80 \\
         \textcolor{cyan}{\textbf{TO-LSTM}} & \textbf{37.79} $\pm$ 6.11 & \textbf{7.64} $\pm$ 0.79 & \textbf{73.99} $\pm$ 3.14 & \textbf{21.06} $\pm$ 1.99 & \textbf{4.95} $\pm$ 1.80 \\
         \midrule
         \multicolumn{6}{c}{\textit{Prediction Horizon = 60 minutes}}\\
         \midrule
         \textcolor{cyan}{\textbf{SNN}} & \textbf{48.47} {$\pm$} 10.02 & \textbf{5.12} $\pm$ 1.14 &  \textbf{68.31} $\pm$ 7.13 & \textbf{19.94} $\pm$ 4.88 & \textbf{11.75} $\pm$ 3.40 \\
         \textcolor{cyan}{\textbf{LSTM}} & \textbf{42.30} $\pm$ 7.13 & \textbf{8.76} $\pm$ 1.33 & \textbf{73.62} $\pm$ 3.45 & \textbf{20.32} $\pm$ 2.11 & \textbf{6.05} $\pm$ 1.86\\
         \textcolor{cyan}{\textbf{TO-SNN}} & \textbf{37.79} $\pm$ 6.11 & \textbf{7.64} $\pm$ 0.79 & \textbf{73.99} $\pm$ 3.14 & \textbf{21.06} $\pm$ 1.99 & \textbf{4.95} $\pm$ 1.80 \\
         \textcolor{cyan}{\textbf{TO-LSTM}} & \textbf{37.79} $\pm$ 6.11 & \textbf{7.64} $\pm$ 0.79 & \textbf{73.99} $\pm$ 3.14 & \textbf{21.06} $\pm$ 1.99 & \textbf{4.95} $\pm$ 1.80 \\
         \midrule
         \multicolumn{6}{c}{\textit{Prediction Horizon = 120 minutes}}\\
         \midrule
         \textcolor{cyan}{\textbf{SNN}} & \textbf{48.47} {$\pm$} 10.02 & \textbf{5.12} $\pm$ 1.14 &  \textbf{68.31} $\pm$ 7.13 & \textbf{19.94} $\pm$ 4.88 & \textbf{11.75} $\pm$ 3.40 \\
         \textcolor{cyan}{\textbf{LSTM}} & \textbf{42.30} $\pm$ 7.13 & \textbf{8.76} $\pm$ 1.33 & \textbf{73.62} $\pm$ 3.45 & \textbf{20.32} $\pm$ 2.11 & \textbf{6.05} $\pm$ 1.86\\
         \textcolor{cyan}{\textbf{TO-SNN}} & \textbf{37.79} $\pm$ 6.11 & \textbf{7.64} $\pm$ 0.79 & \textbf{73.99} $\pm$ 3.14 & \textbf{21.06} $\pm$ 1.99 & \textbf{4.95} $\pm$ 1.80 \\
         \textcolor{cyan}{\textbf{TO-LSTM}} & \textbf{37.79} $\pm$ 6.11 & \textbf{7.64} $\pm$ 0.79 & \textbf{73.99} $\pm$ 3.14 & \textbf{21.06} $\pm$ 1.99 & \textbf{4.95} $\pm$ 1.80 \\
         \bottomrule
    \end{tabularx}
\end{table*}

==> tables/results_ph-60.tex <==


\begin{table*}
    \caption{Performances of the pcRNN model for the three experiments, evaluated at a prediction horizon of 60 minutes and on the Ohio (type 1) and IDIAB (type 2) datasets (mean $\pm$ standard deviation across the dataset).}
    \label{table:res_ph60}
    \begin{tabularx}{\linewidth}{C||C|C|C|C|C}
        \toprule
        \multicolumn{6}{c}{\textbf{Prediction Horizon = 60 minutes}}\\
        \toprule
        \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{RMSE}} & \multirow{2}{*}{\textbf{dRMSE}} &  \multicolumn{3}{c}{\textbf{CG-EGA}} \\
        & & &  AP & BE & EP \\
        \midrule
         \multicolumn{6}{c}{\textit{Experiment 1 - c = 0.0 $\pm$ 0.0}}\\
         \midrule
         
         Ohio & 38.95\scriptsize{ $\pm$ 4.15~} & ~1.62\scriptsize{ $\pm$ 0.14~} & 81.47\scriptsize{ $\pm$ 3.93~} & 10.99\scriptsize{ $\pm$ 1.56~} & ~7.53\scriptsize{ $\pm$ 2.73~} \\
        IDIAB & 35.15\scriptsize{ $\pm$ 7.1~~} & ~1.30\scriptsize{ $\pm$ 0.28~} & 86.38\scriptsize{ $\pm$ 4.54~} & ~7.74\scriptsize{ $\pm$ 2.96~} & ~5.88\scriptsize{ $\pm$ 1.88~} \\
        \textbf{All} & \textbf{37.22\scriptsize{ $\pm$ 5.68~}} & \textbf{~1.47\scriptsize{ $\pm$ 0.27~}} & \textbf{83.70\scriptsize{ $\pm$ 4.67~}} & \textbf{~9.51\scriptsize{ $\pm$ 2.82~}} & \textbf{~6.78\scriptsize{ $\pm$ 2.30~}} \\
        
        \midrule
        
        
         
         \multicolumn{6}{c}{\textit{Experiment 2 - c = 450.0 $\pm$ 0.0}}\\
         
         \midrule
         
        Ohio & 37.67\scriptsize{ $\pm$ 3.79~} & ~1.45\scriptsize{ $\pm$ 0.14~} & 84.26\scriptsize{ $\pm$ 4.02~} & ~9.33\scriptsize{ $\pm$ 1.88~} & ~6.41\scriptsize{ $\pm$ 2.54~} \\
        IDIAB &  33.93\scriptsize{ $\pm$ 6.74~} & ~1.15\scriptsize{ $\pm$ 0.23~} & 88.37\scriptsize{ $\pm$ 4.33~} & ~6.27\scriptsize{ $\pm$ 3.09~} & ~5.36\scriptsize{ $\pm$ 1.80~} \\
        \textbf{All} &  \textbf{35.97\scriptsize{ $\pm$ 5.45~}} & \textbf{~1.31\scriptsize{ $\pm$ 0.25~}} & \textbf{86.13\scriptsize{ $\pm$ 4.60~}} & \textbf{~7.94\scriptsize{ $\pm$ 3.04~}} & \textbf{~5.93\scriptsize{ $\pm$ 2.15~}} \\
        
        \midrule
        
        
         
         \multicolumn{6}{c}{\textit{Experiment 3 - c = 1883.79 $\pm$ 534.91}}\\
         
         \midrule
         
        Ohio & 42.66\scriptsize{ $\pm$ 4.29~} & ~1.27\scriptsize{ $\pm$ 0.15~} & 86.30\scriptsize{ $\pm$ 4.41~} & ~8.38\scriptsize{ $\pm$ 2.15~} & ~5.32\scriptsize{ $\pm$ 2.62~} \\
        IDIAB &  39.78\scriptsize{ $\pm$ 6.95~} & ~0.98\scriptsize{ $\pm$ 0.21~} & 89.78\scriptsize{ $\pm$ 4.06~} & ~4.97\scriptsize{ $\pm$ 3.14~} & ~5.25\scriptsize{ $\pm$ 2.05~} \\
        \textbf{All} &  \textbf{41.66\scriptsize{ $\pm$ 5.51~}} & \textbf{~1.14\scriptsize{ $\pm$ 0.24~}} & \textbf{87.88\scriptsize{ $\pm$ 4.72~}} & \textbf{~6.83\scriptsize{ $\pm$ 3.37~}} & \textbf{~5.29\scriptsize{ $\pm$ 2.36~}} \\
        \bottomrule
    \end{tabularx}
\end{table*}
